Fine-Tuning on Diverse Reasoning Chains Drives Within-Inference CoT Refinement in LLMs

Requiring a large language model (LLM) to generate intermediary reasoning steps, known as Chain of Thought (CoT), has been shown to be an effective way of boosting performance. Previous approaches have focused on generating multiple independent CoTs, combining them through ensembling or other post-hoc strategies to enhance reasoning. In this work, we introduce a novel approach where LLMs are fine-tuned to generate a sequence of Diverse Chains of Thought (DCoT) within a single inference step, which is fundamentally different from prior work that primarily operate on parallel CoT generations. DCoT allows LLMs to gain the ability to perform within-inference refinement of reasoning chains without requiring external feedback. Through a rigorous set of experiments spanning a wide range of tasks that require various reasoning types, we show that fine-tuning on DCoT improves performance over the CoT baseline across model families and scales (1.3B to 70B). These improvements are particularly impactful for tasks with a large result state space, such as those involving numeric answers. Our work is also significant because both quantitative analyses and manual evaluations reveal the observed gains stem from the models' ability to refine an initial reasoning chain by generating a second, improved chain within the same inference step, demonstrating previously elusive self-improvement. Our code and data are publicly available at https://github.com/UKPLab/acl2025-diverse-cot.

==> sections/1_introduction_old.tex <==
% \begin{itemize}
%     \item CoT
%     \item cot collection 
%     \item self-consistency
%     \item gap
%     \item proposal
% \end{itemize}

The impressive language understanding capabilities of large language models (LLMs) is shifting the focus of the research community towards more complex tasks such as reasoning. \cite{NEURIPS2022_9d560961} have shown that certain type of prompts can elicit reasoning abilities in LLMs. In particular, chain of thought (CoT) has been particularly successful. This prompting method makes the model generate a sequence of steps that solves an input problem. The success of CoT in reasoning tasks has pushed the community towards creating fine-tuning LLMs on CoTs (cite many papers that fine-tune on 1 task with CoT). Other works extend fine-tuning datasets with CoTs. \citet{chung2024scaling} employs 9 reasoning tasks with CoT and \citet{kim-etal-2023-cot} scales this up to 1,060 tasks with a total of 1.8M CoTs.

Most of the CoT datasets aims to provide as many pairs of \textit{question-CoT} as possible. \citet{kim-etal-2023-cot} discovered that the amount of tasks is more important than the amount of data points per task to augment LLMs with reasoning abilities. Some works show the potential of distilling CoT data from commercial very large language models (vLLMs) to small large language models (sLLMs) 
\citep{ho-etal-2023-large, hsieh-etal-2023-distilling, huang-etal-2023-large} . \citet{ho-etal-2023-large} propose to augment CoT data with \textit{diverse reasoning}, i.e., sampling multiple CoTs given the same input prompt by merely changing the temperature. While they show this data augmentation technique is effective, it does not provide \textit{diverse reasoning} to the models. In each inference step, the model generates one CoT. We posit that some form of explicit \textit{diverse reasoning} in a single inference step can improve the overall behavior of LLMs in reasoning-intensive tasks. Drawing inspiration from divergent thinking, i.e., a mental process to generate as many new ideas as possible to explore a wide range of potential solutions to a problem, we propose \textit{divergent chain of thought} (DivCoT). It consists of generating multiple CoTs in one inference step to come up with a final solution as shown in \Cref{fig:intro}. One of its main benefits compared to the self-consistency is that DivCoT can achieve gains from just generating two CoTs, while self-consistency requires a minimum of three and gains are typically observed from five \citep{wang2023selfconsistency}.


% However, all these works disregard the fact that a question can be solved in multiple ways. We posit that alternative solutions are valuable and can provide complementary points of view that can solidify the reasoning learning. Based on this intuition, we hypothesize that teaching LLMs multiple ways to solve a question can be beneficial for its generalization of the reasoning patterns.

\begin{figure}[t]
\centering
\includegraphics[width=0.47\textwidth]{figures/overview.png}
\caption{Different types of CoT learning and generation. add one inference step}
\label{fig:intro}
\end{figure}


To generate divergent CoTs, we propose to fine-tune LLMs on a series of reasoning tasks where instead of providing a single CoT as target, we provide a sequence of diverse CoTs as targets. In this way, the LLM learns multiple ways to solve a problem. We build a dataset with 8K questions from 9 popular reasoning tasks and provide diverse CoTs for each question. We build the CoTs using a state-of-the-art commercial LLM and generate multiple independent CoTs per question. Then, we instruction-tuned multiple LLMs of different families and sizes on this dataset and compare it with fine-tuning on vanilla CoT.

In our experiments we show that generating multiple CoTs per question in a single inference step improves the reasoning abilities of LLMs in-domain tasks and in unseen tasks compared to models trained on the same amount of data but generating only one CoT. We observe that performance increase as we increase $k$. Moreover, we find a side-effect from the training in DivCot: LLMs learn to self-correct without any external signal and without being trained to do so. The performance of all our models increases significantly on most datasets when generating two CoTs compared to only one. From our human analysis we confirm that the second CoT usually corrects the first CoT and this is the cause of the performance increase. However, we also observe an \textit{overthinking} effect, when we prompt the model to generate four CoTs. The overall performance of the model is degrades a bit when generating too many CoT. We find the sweet spot on two and three CoTs depending on the model.

Our contributions are as follows:
\begin{itemize}
    \item Divergent Chain of thought (DivCoT), a new CoT method that generates diverse CoTs in one inference step.
    \item A comprehensive set of quantitative and qualitative experiments that show the effectiveness of generating multiple CoTs in one inference step.
    \item The first training method that equip LLMs with self-correct abilities without external feedback.
    \item A new CoT dataset where each question has multiple alternative solutions.
    \item A series of instruction-tuned LLMs on reasoning intensive tasks.
\end{itemize}


% build a large instruction-tuning dataset composed of CoTs with the goal of equipping small LLMs with CoT abilities. They further show that intruction-tuning LLMs on CoT also improves the reasoning abilities of these models on unseen tasks in zero-shot scenarios. CoT can be extended with other methods, such as self-consistency, to improve its performance further. This method consists of sampling multiple alternative responses to a prompt. This allows to obtain multiple CoTs to answer a question and thanks to this its possible to aggregate them to achieve a better answer.

% Inspired by these ideas, we wonder whether instruction-tuning an LLM on multiple alternative CoTs can further improve its reasoning abilities. In other words, our research question is: \textit{does learning how to solve a problem in multiple ways improve the reasoning abilities of an LLM?} We posit that the reasoning abilities of LLMs comes from the reasoning patterns learned during the pertaining phase and hypothesize that the size of a dataset does not necessarily correlate with the number of reasoning patterns, and instead, it is more efficient and effective to provide multiple alternative solutions (i.e., CoTs) to each question in a dataset.





==> sections/6.X_ccot1_improves.tex <==
\Cref{tab:ccot1} doesn't give concluding results of whether CCoT@1 is better or worse than just CoT. This is somewhat expected as both methods are trained on the same data, so CCoT can only show improvements when asking to generate more than 1 CoT.
\input{tables/ccot1}

==> sections/6.X_self_consistency.tex <==
\haritzcomment{move to discussion and remove section}Ensembling methods such as self-consistency usually benefit from generating more candidate answers. In particular, self-consistency generates independent responses and aggregates them with a voting mechanism; therefore, it needs at least three generations to improve performance. Our \texttt{DCoT}, although it may resemble one of them, it is not. Our method generates CoTs that are aware of the previous ones. \Cref{tab:dcot_k} shows that, in general, a $k > 1$ (i.e., the number of generated CoTs) in our \texttt{DCoT} improves the performance of the model across all datasets (compared to $k=1$). Concretely, the best performance of our model is achieved with more than one CoT in 25 cases out of 32 dataset~$\times$~LLM combinations (see \Cref{fig:k_progression} in \Cref{app:dcot_k}). We report the best $k$ for each dataset-LLM on \Cref{tab:bestk} in \Cref{app:bestk}. Moreover, we also observe this behavior in unseen tasks. \Cref{tab:OOD_results} shows that in 8 out of 16 cases, the best performance is obtained by generating more than one CoT. Lastly, we also observe the following interesting behaviors: i) \texttt{DCoT} shows improved performance even in $k=2$. However, this is not the case for self-consistency, where it is impossible to get any gains with $k=2$, and ii) \texttt{DCoT} sometimes exhibits some performance drop when increasing $k$ (e.g., \texttt{Phi-2}@4 on GSM8K). We attribute this to an \textit{overthinking} effect, where the model tries to explore more CoTs and ends up generating wrong CoTs that bias the final answer. Nevertheless, the general improvements by generating more than one CoT confirm the effectiveness of our training method.




% \Cref{tab:dcot_k} shows our \texttt{DCoT} consistently outperforms the baseline with self-consistency (CoT+SC) by a maximum margin of 3.65 and a minimum of 0.88 (average scores across all datasets). Furthermore, \Cref{fig:k_progression} shows that, in general, increasing k improves the performance of the model across all datasets. These results confirm the effectiveness of our CoT training method. Forcing the model to generate multiple CoTs in one inference step enhances performance.





 % These results illustrates that our DSCoT indeed conducts some sort of self-consistency within its parametric knowledge. 


% \Cref{fig:k_progression} shows that in general, increasing k improves the performance of the model. However, we observe that peak performance is usually at $k = 2$ or $3$. Performance at $k=4$ is usually the worse. We attribute this to an \textit{overthinking} effect. These results suggests that the \textit{self-consistency} mechanism learned by the model is different from the original \textit{self-consistency} decoding. In their case, the larger k, the better performance. However, at small k, performance gains are small or even negative. Our model behaves in the opposite way. We obtain gains from $k=2$, making it very cheap to improve performance, but being limitted to small $k$.
% \Cref{tab:self_consistency} shows that CCoT outperforms self-consistency on small models and achieves similar results on large models. This may suggest that CCoT learns to do self-consistency internally in large models and even improves the self-consistency decoding mechanism on small models.

% self-conssitency gives worse results than greedy decoding up to k=4 and only from k=5 yields better results. this improvement make it irregular.

% CCoT makes improvements in a more smooth way.

% \textit{Can self-consistency improve on CCoT?} if not, we can claim self-consistency is being done implicitly inside the parametric knowledge of the model.

% \textit{Self-Consistency is not our rival. We just want to show that our model is doing self-consistency internally. It's difficult to be better than self-consistency because SC is cheaper and easier. No need for new training. More scalable.}

==> sections/6.X_self_correct.tex <==
\textit{Self-correction} is the ability of an LLM to correct its initial response without relying on external feedback \citep{huang-etal-2023-large}. According to them, truly intrinsic self-correction is yet to be found in LLMs.
% Intrinsic self-correction refers to the ability of an LLM to revise or correct its initial response using only its inherent capabilities without relying on external feedback. As previously discussed, recent work suggests that truly intrinsic self-correction is yet to be found in LLMs. 
Our findings show that DCoT-tuned models, trained to generate a multiple CoTs where subsequent CoTs can provide different answers, \emph{do} have the capacity to self-correct initial CoT answers without external feedback, a result of particular note since they are not explicitly trained to do so. In this section, we provide a detailed empirical and careful manual analysis to quantify this effect and understand why it is a form of self-correction.

% Our findings show that DCoT-tuned models can intrinsically self-correct, as demonstrated by their ability to refine and correct their answers generated in the initial chain of thought when generating subsequent chains.
% In this section, we provide a detailed empirical and careful manual analysis to support this finding.

\subsection{Quantitative Analysis of Self-Correction}
In the previous sections, we have demonstrated that \texttt{DCoT} does indeed improve performance. However, these gains could be achieved in two distinct ways: it could be a result of \textit{self-ensembling} \edit{}{of CoTs} as in the case of self-consistency, or alternatively, it could be a result of \edit{\textit{self-correction}}{the refinement of the first answer}. To test which of these mechanisms leads to improvements, we compare the performance of \texttt{DCoT} when we generate two reasoning chains ($k=2$) to that where we generate just one. Importantly, any performance improvement between these cases cannot be a result of self-consistency as two outputs are not sufficient to provide a majority vote, and at least three reasoning chains are needed. For this reason, we only compare DCoT@1 vs DCoT@2, and we do not compare with DCoT@3 or 4.

We can see in \Cref{tab:self_correct} that all models improve performance for most datasets by generating two CoTs instead of one. Specifically, in over 62\% of cases (i.e., 25 out of 40 LLM $\times$ dataset). Furthermore, we can observe performance improvements greater than 0.5 for more than half of the datasets for Phi 1.5, Phi2, LLaMA2 13B, and 70B. This result \edit{is significant because it}{} means that generating a second CoT is beneficial. In other words, the second CoT \textit{overrides} the first, leading to the observed performance gains. %This is fundamentally different from polling, where at least three CoTs are needed.
\edit{We observe a similar effect on the unseen tasks in \Cref{tab:OOD_results}, although the effect is less pronounced due to lower overall improvements on these out-of-domain tasks. Regardless, across models and tasks, we find that in 6/16 cases \haritz{(i.e., models $\times$ tasks)}, \texttt{DCoT@2} improves over \texttt{DCoT@1}, and in 8/16 \texttt{DCoT@k} for \mbox{$k > 1$} improves over \texttt{DCoT@1}, with an additional two cases where the drop with increased $k$ is only marginal.}{} 

These results indicate that DCoT tuning enables models to self-correct. Notably, our training data includes only reasoning chains that lead to the correct answer, never incorrect ones. This suggests that the ability to self-correct can be enabled in LLMs without explicitly training for it.

%We conducted a manual analysis (more detailed in \Cref{sec:human_analysis}) to interpret why we obtain gains by simply generating a second CoT. We observed that the second CoT provides a different reasoning pattern that leads to a different answer, and because of this, the model selects the second answer as the final answer. \Cref{fig:intro} shows an example we found on LLaMA2 7B. This behavior explains the performance gains obtained at $k=2$ and points out that the model is conducting some sort of \textit{self-correction} because by just generating a second CoT without any external feedback, the model changes its final answer and leads to improved performance. This result is extraordinary because \citet{huang2023large} argues that LLMs cannot self-correct yet without any external feedback. Therefore, our work is the first one to achieve this ability without such external feedback, and this is accomplished without any training signal for self-correction. In the next section, we conduct a human analysis to confirm this quantitative observation.





%Furthermore, we can observe performance improvements greater than 0.5 on 6 out of 8 datasets for Phi 1.5, 5/8 for Phi 2, 3/8 on LLaMA 7B, and 6/8 for LLaMA 13B. Notably, all models demonstrate improvements on the GSM8K dataset, which involves math reasoning. 

% Similarly, we also observe a similar effect on the unseen tasks in \Cref{tab:OOD_results}. Although improvements @2 are more difficult to obtain since these are new tasks, and therefore, the model has more difficulty in generating correct CoTs, in 6/16 cases, \texttt{DCoT@2} improves over \texttt{DCoT@1}, and in 8/16 \texttt{DCoT@k} for \mbox{$k > 1$} improves over \texttt{DCoT@1}.

% It is important to emphasize that self-consistency decoding cannot achieve improvements from generating two CoTs because their gains are based on a voting mechanism. However, our method can yield significant improvements without such a voting mechanism. Based on this and the results from \Cref{sec:6_self_consistency}, we argue that our \texttt{DCoT} is conducting some sort of \textit{self-correction} because by just generating a second CoT without any external feedback, the model changes its final answer and leads to improved performance. This result is extraordinary because \citet{huang2023large} argues that LLMs cannot self-correct yet without any external feedback. Therefore, our work is the first one to achieve this ability without such external feedback, and this is accomplished without any training signal for self-correction. In the next section, we conduct a human analysis to confirm this quantitative observation.



==> tables/bbh_perplexity.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\centering
\begin{tabular}{@{}llc@{}}
\toprule
\textbf{LLM}                             & \textbf{Method} & \textbf{Avg}   \\ \midrule
\multirow{2}{*}{Phi 1.5}        & CoT        & 23.35 \\
                                & DCoT     & 25.24 \\\midrule
\multirow{2}{*}{Phi 2}          & CoT        & 22.89 \\
                                & DCoT     & 22.28 \\\midrule
\multirow{2}{*}{LLaMA 7B}       & CoT        & 28.58 \\
                                & DCoT     & 25.75 \\\midrule
\multirow{2}{*}{LLaMA 13B}      & CoT        &   31.95    \\
                                & DCoT     &     28.87  \\\bottomrule
\end{tabular}
\caption{Evaluation on BBH without CoT generation. \haritzcomment{remove?}}
\label{tab:bbh_perplexity}
\end{table}

==> tables/ccot1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{LLM}                             & \textbf{Method} & \textbf{CCoT Gains}                     \\\midrule
\multirow{2}{*}{Phi 1.5}        & DCoT    & \multirow{2}{*}{1.71}   \\
                                & DSCoT@1 &                                \\
\multirow{2}{*}{Phi 2}          & DCoT    & \multirow{2}{*}{-1.14}  \\
                                & DSCoT@1 &                                \\
\multirow{2}{*}{LLaMA 7B}       & DCoT    & \multirow{2}{*}{1.29}   \\
                                & DSCoT@1 &                                \\
\multirow{2}{*}{LLaMA 13B}      & DCoT    & \multirow{2}{*}{-1.08} \\
                                & DSCoT@1 &                                \\
\multirow{2}{*}{LLaMA 13B Chat} & DCoT    &                                \\
                                & CCoT@1 &   
\\\bottomrule
\end{tabular}
\caption{DSCoT@1 vs. DCoT. DSCoT is not significantly better than DCoT when generating only 1 CoT.}
\label{tab:ccot1}
\end{table}

==> tables/datasets.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[h]
% \caption{Brief description of the training datasets.}
% \label{tab:datasets}
\begin{center}
% \scalebox{0.99}{
\setlength{\tabcolsep}{2pt}
% \begin{tabular}{ll}
\begin{tabularx}{\columnwidth}{X|X}
\toprule
\textbf{Dataset}       & \textbf{Reasoning Type}       \\ \midrule
ARC   \citep{clark2018think}        &  Science       \\
BGQA  \citep{kazemi2023boardgameqa}        & Logic                        \\
CoinFlip    \cite{NEURIPS2022_9d560961}  & State-tracking                \\
CondQA (CQA; \citealt{sun-etal-2022-conditionalqa}) & Conditional               \\
GSM8K    \citep{cobbe2021training}     & Math                           \\
HotpotQA  (HQA; \citealt{yang-etal-2018-hotpotqa})    & Explicit multi-hop           \\
LLC    \citep{NEURIPS2022_9d560961}       & Symbolic                   \\
Quartz   \citep{tafjord-etal-2019-quartz}     & Relationships   \\
StrategyQA (StrQA; \citealt{geva-etal-2021-aristotle})    & Implicit multi-hop    \\ \bottomrule
\end{tabularx}
% \end{tabular}
% }
\end{center}
\caption{Brief description of the training datasets.}
\label{tab:datasets}
\end{table}

==> tables/gpt40.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\centering
\begin{tabular}{@{}llll@{}}
\toprule
\textbf{Method (GPT 4o)} & \textbf{SVAMP}          & \textbf{ARC}            & \textbf{Quartz}         \\ \midrule
CoT             & \textbf{83.00} & \textbf{95.28} & \textbf{92.19} \\
DCoT@2          & 80.00          & 91.84          & 90.88          \\ \bottomrule
\end{tabular}
\caption{Preliminary experiments with prompting.}
\label{tab:gpt4o}
\end{table}

==> tables/main_results_old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}



\begin{table*}[t]
% \caption{Comparison of \texttt{DCoT} against \texttt{CoT} on the test sets. *70B results on the dev set.}
% \label{tab:main_results}
\begin{center}
\scalebox{0.87}{
\begin{tabular}{@{}llc|cccccccc@{}}
\toprule
\textbf{LLM}                             & \textbf{Method} & \textbf{Avg.} & \textbf{ARC}   & \textbf{BGQA}  & \textbf{CQA} & \textbf{GSM8K} & \textbf{HQA} & \textbf{LLC}   & \textbf{Quartz} & \textbf{StrQA} \\ \midrule
& CoT      & 47.20    & 48.70 & 32.39 & 61.21         & 34.95 & 32.56    & \textbf{41.00} & 72.69  & 54.08     \\
Phi 1.5                                  & DCoT (Ours)   & \textbf{49.39}   & \textbf{50.01} & \textbf{38.60} & \textbf{62.48} & \textbf{36.85} & \textbf{34.81}    & 39.00 & \textbf{77.39}  & \textbf{55.97}  \\\cmidrule(l){2-11} 
(1.3B)                                & CoT + SC & 46.48	& \textbf{53.81} &	21.59&	63.39&	\textbf{40.33}&	33.63&	32.00&	75.11&	51.96       \\ 
                                & DCoT + SC &   \textbf{49.01}&	53.24&	\textbf{27.60}	&\textbf{65.23}	&40.18&	\textbf{37.79}&	31.00&	\textbf{81.08}&	\textbf{55.97}     \\\midrule
   & CoT      & 60.85    & 70.87 & 39.48 & 65.13         & 56.71 & 52.65    & 58.00 & 82.91  & \textbf{61.06}      \\
Phi 2                                 & DCoT   &\textbf{62.60}    & \textbf{73.77} &\textbf{ 47.07} & \textbf{68.61} & \textbf{60.73} & \textbf{55.15}    & 58.00 & \textbf{83.16}  & 54.34      \\\cmidrule(l){2-11}
(2.7B)                                & CoT + SC & 61.50	& 74.36 &	28.99&	68.14&	64.97&	55.82&	55.00&	85.20&	\textbf{59.51}       \\
                                & DCoT + SC &   \textbf{65.12} & 	\textbf{76.06}	& \textbf{44.16}& 	\textbf{70.53}& 	\textbf{68.08}& 	\textbf{58.61}& 	\textbf{66.00}& 	\textbf{86.09}& 	51.43     \\\midrule
      &CoT & 58.97    & 61.63 & \textbf{43.13} & 65.73         & 28.51 & 53.88    & 75.00 & 79.32  & \textbf{64.59}      \\
                                
LLaMA2                                  & DCoT   & \textbf{60.80}    & \textbf{62.70} & 41.91 & \textbf{70.99} & \textbf{29.57} & \textbf{56.26}    & \textbf{82.00} & \textbf{81.37}  & 61.64      \\\cmidrule(l){2-11}
7B                                & CoT + SC &  \textbf{62.90} & 65.98 &	\textbf{46.04}&	69.92&	33.97&	57.05&	81.00&	83.28&	\textbf{65.99}\\
                                & DCoT + SC &           61.09 &	\textbf{68.53}&	28.20&	\textbf{71.36}&	\textbf{36.01}&	\textbf{58.35}&	\textbf{83.00}&	\textbf{84.05}&	59.22      \\\midrule
     & CoT     & 64.39 &	\textbf{71.79}	&42.63	&70.25	&42.53&	60.23&	\textbf{81.00}&	\textbf{84.82} &	61.85\\
LLaMA2                                 & DCoT   &   \textbf{66.18}&	71.41 &	\textbf{50.21}&	\textbf{71.56}&	\textbf{44.28}&	\textbf{63.52}&	80.00 &	83.29&	\textbf{65.16}      \\\cmidrule(l){2-11}
13B                                 & CoT + SC &  66.82 &	74.82 &	40.80&	\textbf{72.72}&	50.27&	62.34&	80.00&	\textbf{85.84}&	67.75       \\
                                & DCoT + SC &   \textbf{68.12} &	\textbf{74.89}&	\textbf{41.27}&	72.61	&\textbf{54.51	}&\textbf{65.92}	&\textbf{86.00}&	85.07&	\textbf{64.65} \\
                                 \toprule
                      
LLaMA2  & CoT      & \textbf{64.87}	&70.43&	\textbf{44.39}&	\textbf{71.71}&	42.76&	60.83&	\textbf{78.00}&	84.04&	66.78     \\
13B Chat & DCoT   & 64.62&	\textbf{72.22}&	40.94&	71.59&	\textbf{44.20}&	\textbf{63.87}&	71.00&	\textbf{85.43}&	\textbf{67.68}\\
\toprule
LLaMA2 & CoT      &   66.96&	81.69&	\textbf{44.34}&	\textbf{73.59}&	56.00&	\textbf{55.94}&	76.00&	81.99&	66.15    \\
70B* & DCoT   &   \textbf{68.63}&	\textbf{89.04}&	38.30&	69.57&	\textbf{66.00}&	49.78&	\textbf{82.00}&	\textbf{85.99}&	\textbf{68.34} \\      
\bottomrule
\end{tabular}
}
\end{center}
\caption{Comparison of \texttt{DCoT} against \texttt{CoT} on the test sets. *70B results on the dev set.}
\label{tab:main_results}
\end{table*}

==> tables/ood_results_avg.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{multirow}
% \begin{table}[]
% \begin{tabular}{@{}llcccc@{}}
% \toprule
% \textbf{LLM}                        & \textbf{Method} & \textbf{AQuA}           & \textbf{CSQA}           & \textbf{SVAMP}      & \textbf{kLC}    \\ \midrule
% \multirow{2}{*}{Phi 1.5}   & CoT    & 20.27          & 33.88          & 40.00     &      \\
%                            & DCoT   & \textbf{22.38} & \textbf{34.73} & \textbf{40.50} & \\\midrule
% \multirow{2}{*}{Phi 2}     & CoT    & 29.52          & 44.29          & 55.00      &     \\
%                            & DCoT   & \textbf{34.86} & \textbf{45.99} & \textbf{60.50} & \\\midrule
% LLaMA2 & CoT    & \textbf{19.41} & 38.41          & 39.50    &       \\
% 7B     & DCoT   & 17.70          & \textbf{40.79} & \textbf{43.00}&  \\\midrule
% LLaMA2  & CoT    & \textbf{24.85} & 46.55          & \textbf{62.50} & \\
% 13B     & DCoT   & 23.98          & \textbf{47.42} & 56.50& \\         \bottomrule 
% \end{tabular}
% \caption{DCoT vs. CoT on unseen tasks.}
% \label{tab:OOD_results}
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[t]
% \caption{\texttt{DCoT} vs. \texttt{CoT} on unseen tasks.}
% \label{tab:OOD_results}
\begin{center}
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{LLM}                      & \textbf{Method} & \textbf{Avg.}         \\ \midrule
\multirow{5}{*}{Phi 1.5} & CoT    & 32.44±8.51  \\
                         & DCoT@1 & 29.87±8.37  \\
                         & DCoT@2 & 27.29±7.19  \\
                         & DCoT@3 & 29.25±4.86  \\
                         & DCoT@4 & 29.57±5.38  \\ \midrule
\multirow{5}{*}{Phi 2}   & CoT    & 45.70±11.82 \\
                         & DCoT@1 & 49.48±12.15 \\
                         & DCoT@2 & 48.78±12.01 \\
                         & DCoT@3 & 48.86±12.89 \\
                         & DCoT@4 & 49.02±11.28 \\ \midrule
\multirow{5}{*}{LLaMA2}  & CoT    & 33.03±9.30  \\
                         & DCoT@1 & 34.04±11.05 \\
                         & DCoT@2 & 35.17±12.01 \\
                         & DCoT@3 & 34.34±11.91 \\
                         & DCoT@4 & 33.46±10.91 \\ \midrule
\multirow{5}{*}{LLaMA2}  & CoT    & 44.78±15.43 \\
                         & DCoT@1 & 42.40±13.11 \\
                         & DCoT@2 & 42.25±13.65 \\
                         & DCoT@3 & 44.26±16.13 \\
                         & DCoT@4 & 44.27±14.51 \\ \bottomrule
\end{tabular}
\end{center}
\caption{\texttt{DCoT} vs. \texttt{CoT} on unseen tasks.}
\label{tab:OOD_results}
\end{table}

==> tables/self_consistency_old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\begin{tabular}{@{}llc@{}}
\toprule
\textbf{Model}             & \textbf{Method} & \textbf{Avg} \\ \midrule
\multirow{3}{*}{Phi 1.5}   & MCoT  + SC     &              \\
                           & DCoT  + SC     & 47.96       \\
                           & DSCoT           & \textbf{51.61}        \\ \midrule
\multirow{3}{*}{Phi 2}     & MCoT + SC      &              \\
                           & DCoT  + SC     & 63.14        \\
                           & DSCoT           & \textbf{65.22}        \\\midrule
\multirow{3}{*}{LlaMA 7B}  & MCoT  + SC     &              \\
                           & DCoT  + SC     & 62.39        \\
                           & DSCoT           & \textbf{63.27}        \\\midrule
\multirow{3}{*}{LLaMA 13B} & MCoT + SC    &              \\
                           & DCoT + SC     & 67.39        \\
                           & DSCoT         & \textbf{68.96}       
\\\bottomrule
\end{tabular}
\caption{self-consistency. We use up to 4 CoTs/question}
\label{tab:self_consistency}
\end{table}

==> tables/self_correct.tex <==
% \begin{table*}[b]
% \caption{Performance gain from generating two CoTs instead of one on the dev set.}
% \label{tab:self_correct}
% \begin{center}
% \begin{tabular}{@{}lcccccccc@{}}
% \toprule
% \textbf{LLM}     & \textbf{ARC}         & \textbf{BGQA}         & \textbf{CQA} & \textbf{GSM8K} & \textbf{HQA}     & \textbf{LLC} & \textbf{Quartz}      & \textbf{StrQA}    \\\midrule
% Phi 1.5   & 1.26 $\uparrow$  & 2.10 $\uparrow$ & 0.10          & 3.00 $\uparrow$  & 0.83 $\uparrow$    & -14.00  $\downarrow$ & 3.38 $\uparrow$  & 1.11  $\uparrow$     \\
% Phi 2     & -3.56 $\downarrow$ & -2.38 $\downarrow$ & 0.95  $\uparrow$        & 0.80 $\uparrow$  & 1.06 $\uparrow$    & 14.00 $\uparrow$  & 1.55 $\uparrow$  & -0.85 $\downarrow$     \\
% LLaMA2 7B  & 1.28 $\uparrow$  & -0.99 $\downarrow$ & -0.56  $\downarrow$       & 4.00 $\uparrow$ & -0.01    & 6.00  $\uparrow$ & -1.04 $\downarrow$ & 0.25       \\
% LLaMA2 13B & 4.15 $\uparrow$  & 0.91 $\uparrow$  & -1.02  $\downarrow$       & 3.00 $\uparrow$ & 2.02  $\uparrow$   & 12.00 $\uparrow$ & 0.77 $\uparrow$  & -2.03 $\downarrow$ \\
% LLaMA2 70B & 3.24 $\uparrow$  & 1.38 $\uparrow$  & 3.68  $\uparrow$       & 10.00 $\uparrow$ & 0  & 4.00 $\uparrow$ & -1.00 $\downarrow$  & -4.07 $\downarrow$ \\\bottomrule
% \end{tabular}
% \end{center}
% % \caption{Performance gain from generating two CoTs instead of one on the dev set.}
% % \label{tab:self_correct}
% \end{table*}


\begin{table*}[b]
\centering
\begin{tabular}{@{}lcccccccc@{}}
\toprule
\textbf{LLM} & \textbf{ARC} & \textbf{BGQA} & \textbf{CQA} & \textbf{GSM8K} & \textbf{HQA} & \textbf{LLC} & \textbf{Quartz} & \textbf{StrQA} \\ \midrule
Phi 1.5 & \cellcolor{green!20}1.26 & \cellcolor{green!30}2.1 & \cellcolor{green!1}0.1 & \cellcolor{green!40}3 & \cellcolor{green!20}0.83 & \cellcolor{red!50}-14 & \cellcolor{green!40}3.38 & \cellcolor{green!20}1.11 \\ \midrule
Phi 2 & \cellcolor{red!30}-3.56 & \cellcolor{red!20}-2.38 & \cellcolor{green!20}0.95 & \cellcolor{green!20}0.8 & \cellcolor{green!20}1.06 & \cellcolor{green!50}14 & \cellcolor{green!30}1.55 & \cellcolor{red!10}-0.85 \\ \midrule
LLama2 7B & \cellcolor{green!20}1.28 & \cellcolor{red!10}-0.99 & \cellcolor{red!10}-0.56 & \cellcolor{green!40}4 & -0.01 & \cellcolor{green!40}6 & \cellcolor{red!10}-1.04 & \cellcolor{green!10}0.25 \\ \midrule
LLama2 13B & \cellcolor{green!40}4.15 & \cellcolor{green!20}0.91 & \cellcolor{red!10}-1.02 & \cellcolor{green!40}3 & \cellcolor{green!20}2.02 & \cellcolor{green!50}12 & \cellcolor{green!20}0.77 & \cellcolor{red!20}-2.03 \\ \midrule
LLama2 70B & \cellcolor{green!30}3.24 & \cellcolor{green!30}1.38 & \cellcolor{green!40}3.68 & \cellcolor{green!50}10 & 0 & \cellcolor{green!40}4 & \cellcolor{red!10}-1 & \cellcolor{red!40}-4.07 \\ \bottomrule
\end{tabular}
\caption{Performance gain from generating two CoTs instead of one on the dev set.}
\label{tab:self_correct}
\end{table*}
